On the Impact of Dark Matter Scattering on the Trajectory of High-Energy Cosmic Rays

We study the impact on the trajectory of high-energy cosmic-ray protons of scattering off the cosmic dark matter. We compute the scattering angle as a function of the cosmic-ray energy, of the dark matter mass, and of the interaction strength for a few representative choices for the relevant interaction cross section. We find that the typical deflection angle over the cosmic ray path is largely independent of the dark matter mass. Given existing limits on the interaction strength, we compute the average deflection angle. We find that for large interaction cross sections and low cosmic ray energies, the predicted deflection angle is much larger than the angular resolution of very high-energy cosmic-ray observatories such as Pierre Auger.

==> sections/old_notes.tex <==




\SP{We may need to rephrase this once we understand the H.E. structure of the various operators} We consider a sample of four effective operators, producing four different and representative structures in the non-relativistic limit. In particular, we include both spin-dependent and spin-independent operators, and velocity dependent and velocity-independent operators. Specifically, we consider:
\begin{itemize}
    \item scalar-scalar (SS): $\bar\chi\bar q q$: this operator is spin-independent and velocity-independent (leading operator in the non-relativistic limit: 1);
    \item axial vector-axial vector (AVAV): $\bar\chi \gamma^5 \gamma^\mu \chi\bar q\gamma^5\gamma_\mu q$: this operator is spin-dependent, but velocity independent (leading operator in the non-relativistic limit: $\vec s_\chi\cdot \vec s_N$);
    \item pseudoscalar-pseudoscalar (PSPS): $\bar\chi\gamma^5 \chi\bar q\gamma^5 q$: this operator is both spin-dependent and momentum-dependent (leading operator in the non-relativistic limit: $(\vec s_\chi\cdot \vec q)(\vec s_N\cdot \vec q)$);
    \item vector-axial vector (VAV): $\bar\chi\gamma^\mu\chi\bar q\gamma_\mu\gamma^5 q$: this operator is spin-dependent and velocity dependent (leading operator in the non-relativistic limit: $\vec s_N^\perp\cdot\vec v$).
\end{itemize}

\SP{Grant: can we check if we get anything different with other operators?}

We are primarily concerned with the scattering of light dark matter off of nucleons. The most stringent constraints arise from up-scattered dark matter particles from dark matter-cosmic-ray scattering, in XENON 1T and MiniBOONE \cite{Bringmann:2018cvk}; the gap between these constraints was filled with Daya Bay data in Ref.~\cite{Cappiello:2019qsw}. At about 0.1 GeV, stronger constraints arise from the XENON10, XENON100, and XENON 1T experiments (see e.g. Fig.~1 in Ref.~\cite{Essig:2022dfa}). Below 0.1 GeV, the limits on the dark matter-nucleon %spin-independent
cross section are roughly around a few times $10^{-31}\ {\rm cm}^2$, roughly independent of mass; here, conservatively, we take $10^{-31}\ {\rm cm}^2$ as the typical constraint

%For reference







\section{Kinematics Calculation}

\noindent In 3D space, the collision takes place in the x-direction, $\theta$ is the scattering angle in the center of mass frame and $\theta^*$ is the scattering angle in the laboratory frame. 

\vspace{1 cm}
\begin{multicols}{2}
\begin{figure}[H]
\centering
\begin{tikzpicture}[
roundnode/.style={circle, minimum size=0mm},
squarednode/.style={rectangle, minimum size=7mm},
]
%Nodes
\node[roundnode] (2)                          {$p_2^C$};
\node[roundnode] (c)      [right=15mm of 2]   {};
\node[roundnode] (1)      [right=15mm of c]   {$p_1^C$};
\node[roundnode] (3)      [above=of 1]        {$p_3^C$};
\node[roundnode] (4)      [below=of 2]        {$p_4^C$};
\node[roundnode] (temp)   [left=6mm of 1]     {};
\node[roundnode] (a*)     [above=0.1mm of temp]  {$\theta$};
\node[squarednode](title) [above=20 mm of c, font=\bfseries]{
Center Of Mass Frame};
%Lines
\draw[->]   (2) -- (c);
\draw[->]   (1) -- (c);
\draw[->]   (c) -- (3);
\draw[->]   (c) -- (4);
%Arc/Angle
\draw (28mm,0mm) arc (0:33.69:7.5mm);
\end{tikzpicture} 
\end{figure}

\noindent 4-momentum in center of mass frame
\begin{align*}
    &p_1^C = \left(E_1,\ -p,\ 0,\ 0 \right), \\
    &p_2^C = \left(E_2, \ +p, \ 0, \ 0\right). \\
    &p_4^{C} = \left({E_4, \ - p \cos{(\theta})}, \ -p \sin {(\theta)}, \ 0\right), \\
    &p_3^{C} = \left({E_3, \ p \cos{(\theta)}}, \ p \sin {(\theta)}, \ 0\right).
\end{align*}
\vspace{0.25cm}

\noindent 4-momentum after Lorentz boost:
\begin{align*}
    &p_1^{C'} = \left(\gamma \left(E_1 - \beta p \right), \ \gamma \left( -p + \beta E_1\right), \ 0, \ 0\right), \\
    &p_2^{C'} = \left(\gamma \left(E_2 + \beta p \right),\ \gamma \left( p + \beta E_2\right),\ 0,\ 0 \right), \\
    &p_4^{C'} = \left(\gamma \left(E_4 - \beta p \cos{(\theta)}\right), \ \gamma \left(-p\cos{(\theta)} + \beta E_4\right), \ -p \sin{(\theta)}, \ 0\right), \\
    &p_3^{C'} = \left(\gamma \left(E_3 + \beta p\cos{(\theta)} \right), \ \gamma \left(p \cos{(\theta)} + \beta E_3\right), \ p \sin {(\theta)}, \ 0\right).
\end{align*}
\columnbreak
\begin{figure}[H]
\centering
\begin{tikzpicture}[
roundnode/.style={circle, minimum size=0mm},
squarednode/.style={rectangle, minimum size=7mm},
]
%Nodes 
\node[roundnode] (2)                         {$p_2^L$};
\node[roundnode] (c)   [right=15mm of 2]     {$p_1^L$};
\node[roundnode] (1)   [right=15mm of c]     {};
\node[roundnode] (3)   [above=12mm of 1]     {$p_3^L$};
\node[roundnode] (4)   [below=12mm of 1]     {$p_4^L$};
\node[roundnode] (temp)[right=4mm of c]      {};
\node[roundnode] (a)   [above=0.1mm of temp] {$\theta^*$};
\node[squarednode](title)[above=20mm of c, font=\bfseries]{
Laboratory Frame};
%Lines
\draw[->]      (2) -- (c);
\draw[->]      (c) -- (3);
\draw[->]      (c) -- (4);
\draw[dashed]  (c) -- (1);
%Arc/Angle
\draw (32mm,0mm) arc (0:33.69:9mm);
\end{tikzpicture}
\end{figure}

\noindent In the laboratory frame, the 4-momentum before collision
\begin{align*}
    &p_1^L = \left(m_1, \  0, \  0, \ 0 \right), \\
    &p_2^L = \left(E_2,\ p_L,\ 0 ,\ 0\right). \\
    &p_3^{L} = \left(E_3, \ p_L \cos{(\theta^*)}, \ p_L \sin{(\theta^*)}, \ 0 \right), {\rm incorrect}\\
\end{align*}
\end{multicols}

\noindent{Calculating p, from Lorentz boosted CM frame and Lab frame of dark matter}
\begin{align*}
    &\gamma(-p + \beta E_1) = 0 \\
    &p = \beta E_1
\end{align*}

\noindent{Calculating $\beta$ and $\gamma$,}

\begin{align*}
    &\vec{p_{tot}^L} = (E_2 + m_1, \sqrt{E_2^2 - m_2^2}), \\
    &\vec{p_{tot}^C} = 0, \\
    &\vec{p_{tot}^C} = \vec{p_{tot}^{L'}}, \\
    &\gamma(p_{tot} - \beta E_) = 0, \\
\end{align*}
\begin{equation}
   \beta = \frac{\sqrt{E_2^2 - m_2^2}}{E_2 + m_1} \And \gamma = \frac{1}{\sqrt{1-\beta^2}}
\end{equation}

\noindent Using 3-momenta of the nucleon after collision, to relate CM and Lab angles
\begin{align*}
    &p_3^{C'} = p_3^{L}, \\
    & \left(\gamma \left(p \cos{(\theta)} + \beta E_3\right), \ p \sin {(\theta)}, \ 0\right) = \left(p_L \cos{(\theta^*)}, \ p_L \sin{(\theta^*)}, \ 0 \right)
\end{align*}

\noindent Equating momentum in x and in y respectively 
\begin{align*}
    &\gamma\left(p \cos{(\theta)} + \beta E_3\right) = p \cos {(\theta^*)} \\
    &p \sin{(\theta)} = p \sin{(\theta^*)} \\
    &\tan{(\theta}) = \frac{\gamma p_L\sin{(\theta^*)}}{\left(p_L\cos{(\theta^*)} - \gamma\beta E_3\right)} \\
    &\cos{(\theta)} = \frac{1}{\sqrt{1 + \frac{\gamma^2 p_L^2 \sin^2{(\theta^*)}}{(\gamma \beta E_3  - p_L\cos{(\theta^*)})^2}}} \\
    & \text{where} \ p_L = \gamma(p + \beta E_2)
\end{align*}



\noindent From Eqn 4 of Dick and Norbury (2009), where $\theta^*$ is the angle in the Lab frame and $\theta$ is the angle in the CM frame. $d\Omega$ refers to the solid angle in the CM frame and $d\Omega^*$ refers to the solid angle in the Lab frame. 
\begin{equation}
    \left(\frac{d\sigma}{d\Omega^*}\right) = \left| \frac{d\cos{(\theta)}}{d\cos{(\theta^*)}} \right| \left(\frac{d\sigma}{d\Omega}\right)
\end{equation}

\noindent The inverse of the derivative of Eqn 41 with respect to $\cos{\theta}$ gives the kinematic factor $f$, linking the CM frame and Lab frame.

\begin{equation}
    f = \left|\frac{d\cos{(\theta)}}{d\cos{(\theta^*)}}\right| = 
    \frac{\gamma^2 p_L^3 \sin^2{(\theta^*)}}
    {\left(p_L\cos{(\theta^*)- \gamma \beta E_3}\right)^3
    \left(1 + \frac{\gamma^2 p_L^2 \sin^2{(\theta^*)}}
    {\left(\gamma \beta E_3  - p_L\cos{(\theta^*)}\right)^2}\right)^{\frac{3}{2}}}
\end{equation}

Notice that the Mandelstam variables, expressed in terms of kinematic variables in the Lab frame, read:
\begin{equation}
    s=(m_1+E_2)^2-p_L^2;
\end{equation}
\begin{equation}
    t=(E_3-E_2)^2-2p_L^2(1-\cos\theta^*)
\end{equation}




